Captured by Captions: On Memorization and its Mitigation in CLIP Models

Multi-modal models, such as CLIP, have demonstrated strong performance in aligning visual and textual representations, excelling in tasks like image retrieval and zero-shot classification. Despite this success, the mechanisms by which these models utilize training data, particularly the role of memorization, remain unclear. In uni-modal models, both supervised and self-supervised, memorization has been shown to be essential for generalization. However, it is not well understood how these findings would apply to CLIP, which incorporates elements from both supervised learning via captions that provide a supervisory signal similar to labels, and from self-supervised learning via the contrastive objective. To bridge this gap in understanding, we propose a formal definition of memorization in CLIP (CLIPMem) and use it to quantify memorization in CLIP models. Our results indicate that CLIP's memorization behavior falls between the supervised and self-supervised paradigms, with "mis-captioned" samples exhibiting highest levels of memorization. Additionally, we find that the text encoder contributes more to memorization than the image encoder, suggesting that mitigation strategies should focus on the text domain. Building on these insights, we propose multiple strategies to reduce memorization while at the same time improving utility--something that had not been shown before for traditional learning paradigms where reducing memorization typically results in utility decrease.

==> content/ideas.tex <==
What are the things we want to show:
\begin{enumerate}
    \item How CLIP memorization relates to SL and SSL memorization. 1
    \item Which modality (text or vision) is more responsible for memorization? 2
    \item Which samples are memorized and why? 3
    \item How does the CLIP memorization impact generalization? 4
    \item How can we prevent memorization and maybe, at the same time, get better CLIP models? 5
\end{enumerate}


\subsection{What are the results that we currently have:}

Question 0: Overview on CLIPMem results.

Question 1: 

Question 2: 


Question 3: 

Question 4: 

Question 5: 



\subsection{What are the results we are currently still waiting for:}

Question 1: 


Question 2: 
1. Diffusion model results: get 5 generated images and train with them.
2. Multiple training effects:
NONE
- no augmentation for text and image
ONLY IMAGE
- normal crop augmentation for image, no augmentation for text
- diffusion model augmentation for image, no augmentation for text
ONLY TEXT
- no image augmentation and 5 coco captions
- no image augmentation and 5 GPT3 captions
BOTH
- diffusion + 5 coco
- diffusion + GPT3
- crop + + 5 coco
- crop + GPT3


Question 3: 
1. Test if the images that are most memorized when the 5 (diverse) captions are used are still highly memorized when 1 caption is used. This would indicate that CLIP memorizes the most difficult samples (difficulty is measured based on the fact that also human annotators do not agree) 

Question 4: 

Question 5: 
